Going Beyond Feature Similarity: Effective Dataset Distillation based on Class-Aware Conditional Mutual Information

Dataset distillation (DD) aims to minimize the time and memory consumption needed for training deep neural networks on large datasets, by creating a smaller synthetic dataset that has similar performance to that of the full real dataset. However, current dataset distillation methods often result in synthetic datasets that are excessively difficult for networks to learn from, due to the compression of a substantial amount of information from the original data through metrics measuring feature similarity, e,g., distribution matching (DM). In this work, we introduce conditional mutual information (CMI) to assess the class-aware complexity of a dataset and propose a novel method by minimizing CMI. Specifically, we minimize the distillation loss while constraining the class-aware complexity of the synthetic dataset by minimizing its empirical CMI from the feature space of pre-trained networks, simultaneously. Conducting on a thorough set of experiments, we show that our method can serve as a general regularization method to existing DD methods and improve the performance and training efficiency.

==> chapters/rebuttal.tex <==
\section{Rebuttal}

\subsection{Global Response}
We sincerely express our gratitude for dedicating your valuable time to providing insightful suggestions that can enhance our paper. Your praise regarding our methodology, experiments, and contributions have greatly encouraged and motivated us. Our detailed responses to all of your conerns are presented below.

Encouragingly, reviewers praise the insight of using CMI in dataset distillation ( R\#oMQb , R\#kma8 ), solid theoretical foundation ( R\#kma8 ,
R\#zh5i ), robustness ( R\#oMQb , R\#kma8 ) and comprehensive experiments ( R\#oMQb ,
R\#kma8, R\#i6mf, R\#zh5i ) of our work. To better address the reviewers' concerns, we provide point-by-point responses to each reviewer below. If there are any other questions, please don't hesitate to discuss them with us.

\subsection{Reviewer 1}
We sincerely express our gratitude for dedicating your valuable time to providing insightful suggestions that can enhance our paper. Your praise regarding our methodology,
experiments, and contributions have greatly encouraged and motivated us. Our detailed responses to all of your concerns are presented below.

\begin{table}[!ht]
    \centering
    \tabcolsep=10.5pt
    \caption{Additional time consumption (s) per iteration of adding CMI constraint. }
    \label{tab:training_cost}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ll *{6}{c}}
        \toprule
           &  &  \multicolumn{3}{c}{CIFAR10} & \multicolumn{3}{c}{CIFAR100}\\
        \midrule
          & & 1/10 & 1/5 & 1 & 1/10 & 1/5 & 1\\
        \midrule
        \multirow{2}{*}{IDM} & time (s)  & 0.05 & 0.1 & 0.5 & 0.5 & 2.5 & 5\\
         & acc (\%) & 61.9$\pm$0.3 & 62.1$\pm$0.2 & 62.2$\pm$0.3 & 46.7$\pm$0.1 & 47.0$\pm$0.2 & 47.2$\pm$0.4\\
        \midrule
        \multirow{2}{*}{IDC} & time (s) & 0.4 & 0.8 & 4.4 & 3.2 & 6.4 & 32.0\\
         & acc (\%) & 69.6$\pm$0.3 & 70.0$\pm$0.2 & 70.0$\pm$0.3 & 46.0$\pm$0.3 & 46.4$\pm$0.3 & 46.6$\pm$0.3\\
        \bottomrule
    \end{tabular}}
    % \vspace{-1.0em}
\end{table}
\subsubsection{Weakness 1}
\textbf{Balance between training cost and performance}

Thanks for you suggestion on improving the experimental completeness, we conduct experiments on reducing the calculation frequency of CMI constraints as shown in Table below. We report the performance and additional time consumption per iteration under different optimization settings, where the ratio of CMI optimization steps to distillation loss optimization steps is set to 1/10, 1/5, and 1. It can be observed that even under significantly reduced optimization step settings, the CMI constraint still achieves stable performance improvements.

\begin{table}[!ht]
    \centering
    \tabcolsep=10.5pt
    \caption{Performance improvements of CMI constraint on trajectory matching distillation methods.}
    \label{tab:improve_iid_copy}
    \vspace{-2mm}\resizebox{1\linewidth}{!}{
    \begin{tabular}{l *{6}{c}}
        \toprule
          & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{CIFAR100}  \\
            \midrule
        Method  & 10 & 50 & 10 & 50 & 10 & 50 \\
        \midrule
        IID-DM$^\dagger$   & 74.5$\pm$0.2 & 84.0$\pm$0.3  & 52.5$\pm$0.3 & 64.5$\pm$0.4  & 31.5$\pm$0.3 & 43.0$\pm$0.1   \\
        \textbf{DM+CMI}   & \textbf{77.9$\pm$0.4} & \textbf{84.9$\pm$0.4}  & \textbf{52.9$\pm$0.3} & \textbf{65.8$\pm$0.3}  & \textbf{32.5$\pm$0.4} &  \textbf{44.9$\pm$0.2}  \\
        \midrule
        IID-IDM$^\dagger$  & 81.8$\pm$0.1 & 84.7$\pm$0.3  & 59.4$\pm$0.2 & 68.3$\pm$0.2  & 45.8$\pm$0.4 & 51.0$\pm$0.3 \\
        \textbf{IDM+CMI}  & \textbf{84.3$\pm$0.2} & \textbf{88.9$\pm$0.2}  & \textbf{62.2$\pm$0.3} & \textbf{71.3$\pm$0.2}  & \textbf{47.2$\pm$0.4} & \textbf{51.9$\pm$0.3} \\
        \bottomrule
    \end{tabular}}
\end{table}
\subsubsection{Weakness 2}
\textbf{Comparison with other complexity measure}

Compare to other complexity metric which evaluate the complexity of a single data point (e.g., GraDN Score [1]), CMI is a class-based concept, considering all the feature vectors within one class as a whole. On the other hand, CMI enables the computation process to follow a deterministic mathematical expansion, results in a more accurate information metric. Moreover, the insight of minimizing CMI stems from constraining the complexity of the overall synthetic dataset, making it a versatile plugin. Here, we list several information metrics used in previous distillation methods and make a brief summarization:

\textbf{Influence Function [2]. } influence function determines the importance of a sample by comparing the loss difference after removing a specific sample. However, this method requires retraining the model for each sample, leading to a significant computational overhead, making it impractical to optimize. Thus [3] only consider it as a evaluation metric.

\textbf{Mutual Information (MI). } MIM4DD [4] increases the MI between the synthetic and original datasets by incorporating a contrastive learning framework. Although it is not explicitly used for complexity constraints, MI is still an information metric and is thus included in our comparison. 

\textbf{Mean-square Error (MSE). }, IID [5] uses the MSE loss between each sample and its corresponding class center as a regularization, which is applicable only to distribution matching methods. 

\textbf{GraDN Score.}, SDC [6] uses the GraDN Score of the synthetic dataset corresponding to the proxy model during training as a regularization, which is applicable only to gradient matching methods. 

For a more intuitive comparison, we have compared the performance of our work with [4], [5], and [6] as shown in \textbf{Table 1} provided in \textbf{Sec 5.2} and \textbf{Table 8} provided in \textbf{Sec A.1}. We provide an additional comparative experiment where we remove another regularization term (i.e., MSE loss between the variance matrix of the synthetic dataset and that of the real dataset) from IID and compare it with our method in Table below. It can be observed that CMI not only accelerates model training but also achieves better constraint performance across various distillation methods and datasets.

[1] Deep learning on a data diet: Finding important examples early in training. In NeurIPS, 2021.

[2] Understanding black-box predictions via influence functions. In ICML, 2017.

[3] What is Dataset Distillation Learning? In ICML, 2024.

[4] MIM4DD: Mutual Information Maximization for Dataset Distillation. In NeurIPS, 2023.

[5] Exploiting Inter-sample and Inter-feature Relations in Dataset Distillation. In CVPR, 2024.

[6] Not All Samples Should Be Utilized Equally: Towards Understanding and Improving Dataset Distillation. In arXiv, 2024.
 
\begin{table}[!ht]
\centering
\tabcolsep=10.5pt
\caption{Comparison with baseline method SRe$^2$L on various datasets.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{Dataset}       & \multirow{2}{*}{IPC} & \multicolumn{2}{c}{ResNet-18}                          & \multicolumn{2}{c}{ResNet-50}                          & \multicolumn{2}{c}{ResNet-101}                         \\ \cmidrule(l){3-8} 
                               &                      & SRe$^2$L & Ours                                        & SRe$^2$L & Ours                                        & SRe$^2$L & Ours                                        \\ \midrule
\multirow{3}{*}{ImageNet-1K}     & 10  &  21.3$\pm$0.6    & \textbf{24.2$\pm$0.3} & 28.2$\pm$0.4   & \textbf{30.8$\pm$0.5} & 30.5$\pm$0.3    & \textbf{23.0$\pm$0.1}\\
                               & 50                  & 46.8$\pm$0.2     & \textbf{49.1$\pm$0.1} & 55.6$\pm$0.2    & \textbf{58.4$\pm$0.3} & 56.4$\pm$0.3     &  \textbf{58.7$\pm$0.2}\\
                               & 100                  & 52.8$\pm$0.3    &  \textbf{54.6$\pm$0.2}& 61.1$\pm$0.1    & \textbf{63.6$\pm$0.3} & 62.5$\pm$0.2     & \textbf{64.2$\pm$0.3} \\ \midrule
ImageNet-21K & 10                   & 18.5$\pm$0.4    & \textbf{21.6$\pm$0.2} & 27.2$\pm$0.3     & \textbf{29.8$\pm$0.4} & 27.5$\pm$0.1     & \textbf{30.1$\pm$0.2} \\
\bottomrule
\end{tabular}
}
\label{tab:baseline}
\end{table}
\subsubsection{Weakness 3}
\textbf{Experimental results with larger datasets and more complex models}

Thank you for your valuable suggestions regarding enhancing the robustness of the method. We conduct additional experiments on a larger dataset (i.e., ImageNet-21K) and more complex model (e.g., ResNet101) by appling CMI constraint on SRe$^2$L to evaluate the performance of our proposed method. The results shown in Table below demonstrate that our method achieves significant performance improvements under all settings, validating the generality of the proposed method. We will include additional relevant experiments in the final version of the manuscript.

\subsubsection{Question 1}
\textbf{Definition of empirical CMI}

Thank you for your suggestion on improving the presentation in the paper. Here, we propose the term empirical CMI to differentiate it from the CMI formula derived through explicit mathematical expressions in \textbf{Eq. 8}. In practical applications, empirical originates from the estimation of $P_{\hat{Z} \mid Y}$, i.e., using $Q_{\text{emp}}^{Y}$ obtained by summing over all sampled points and averaging as a numerical approximation of $P_{\hat{Z} \mid Y}$. For a specific synthetic dataset $\mathcal{S}_{y} = \{ (\mathbf{s}_{1}, y), (\mathbf{s}_{2}, y), \cdots, (\mathbf{s}_{n}, y) \}$ given $Y = y$, $Q_{\mathrm{emp}}^{y}=\frac{1}{\left|\mathcal{S}_{y} \right|} \sum_{\mathbf{s}_{i} \in \mathcal{S}_{y}} P_{\mathbf{s}_{i}}$. We then use $Q_{\mathrm{emp}}^{y}$ as the numerical estimate of $P_{\hat{Z} \mid Y}$ and substitute it into \textbf{Eq. 8} to calculate the computable CMI value.

\begin{wraptable}{r}{0.6\linewidth}
    \centering
    \caption{ablation of proxy model with DM. }
    \label{tab:dm_abl}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l *{4}{c}}
        \toprule
           & \multicolumn{4}{c}{DM} \\
            \midrule
         & ConvNet & AlexNet & VGG11 & ResNet18\\
        \midrule
        Depth & 3 & 5 & 8 & 17 \\
        Dimensionality & 2048 & 4096 & 512 & 512\\
        Model Acc (\%)  & 79.8 & 80.2 & 79.4 & 79.5\\
        Start CMI value & 0.1045 & 1.9338 & 0.0021 & 0.0016\\
        End CMI value w.o. cstr & 0.0866 & 1.6217 & 0.0059 & 0.0066 \\
        End CMI value w. cstr & 0.0326 & 0.6642 & 0.0006 & 0.0004 \\
        Performance (\%) & 51.2 & 50.8 & 52.4 & 52.9\\
        \bottomrule
    \end{tabular}}
    \vspace{-1.0em}
\end{wraptable}
\subsubsection{Question 2}
\textbf{Ablation study of diverse model architectures}

Thank you for your suggestion on improving the ablation experiments. In \textbf{Table 7}, we present the performance when using ConvNet and ResNet18 as proxy models for calculating CMI. Following your advice, we have conducted more comprehensive ablation experiments. Under the CIFAR10 with IPC=10, we utilized simply pre-trained ConvNet, AlexNet, ResNet18, and VGG11 as proxy models to compute CMI for both DM and DSA.

\begin{wraptable}{r}{0.6\linewidth}
    \centering
    \caption{ablation of proxy model with DSA. }
    \label{tab:dsa_abl}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l *{4}{c}}
        \toprule
           & \multicolumn{4}{c}{DM} \\
            \midrule
         & ConvNet & AlexNet & VGG11 & ResNet18\\
        \midrule
        Depth & 3 & 5 & 8 & 17 \\
        Dimensionality & 2048 & 4096 & 512 & 512\\
        Model Acc (\%)  & 79.8 & 80.2 & 79.4 & 79.5\\
        Start CMI value & 0.1045 & 1.9338 & 0.0021 & 0.0016\\
        End CMI value w.o. cstr & 0.0825 & 1.8755 & 0.0076 & 0.0051 \\
        End CMI value w. cstr & 0.0455 & 0.8875 & 0.0005 & 0.0004 \\
        Performance (\%) & 53.2 & 53.4 & 54.8 & 54.7\\
        \bottomrule
    \end{tabular}}
    \vspace{-1.0em}
\end{wraptable}
We sequentially report the following metrics: the depth (i.e., number of convolution layer), the dimensionality of the feature space, and the accuracy on the original dataset of the proxy model; the start CMI value of the synthetic dataset, the CMI value at the end of the optimization process w.o. and w. CMI constraint (cstr) of the synthetic dataset, and the accuracy of the model trained using the synthetic dataset. As shown in Table below, it can be observed that the dimensionality of the feature space has a greater impact on CMI values than network depth, and CMI effectively reflects the degree of clustering in $\hat{Z}$ under the same dimensional conditions. Nonetheless, the proposed CMI constraint effectively regulates the complexity of the synthetic dataset, demonstrating the strong generalization capability of our approach.

\begin{wraptable}{r}{0.3\linewidth}
    \centering
    % \vspace{-1.5em}
    \caption{federated learning. }
    \label{tab:fed}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c *{2}{c}}
        \toprule
           & \multicolumn{2}{c}{FL} \\
            \midrule
        IPC & DM & DM + CMI\\
        \midrule
        3  & 53.6 & \textbf{54.1} \\
        5 & 62.2 & \textbf{63.0} \\
        10 & 69.2 & \textbf{70.4}\\
        \bottomrule
    \end{tabular}}
    \vspace{-1.0em}
\end{wraptable}
\begin{wraptable}{r}{0.4\linewidth}
    \centering
    % \vspace{-1.5em}
    \caption{Continual learning. }
    \label{tab:cont}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c *{2}{c}}
        \toprule
           & \multicolumn{2}{c}{CL} \\
            \midrule
        Number of Classes & IDC & IDC + CMI\\
        \midrule
        20  & 65.5 & \textbf{67.2} \\
        40 & 61.2 & \textbf{62.4} \\
        60 & 54.5 & \textbf{56.1} \\
        80 & 50.4 & \textbf{53.6} \\
        100 & 46.5 & \textbf{50.2} \\
        \bottomrule
    \end{tabular}}
    \vspace{-1.0em}
\end{wraptable}
\subsubsection{Question 3}
\textbf{Application on downstream tasks}

Thanks for the suggestion. Following your guidance, we explore the proposed method across two downstream tasks commonly used in dataset distillation: federated learning (FL) and continual learning (CL). The experimental results are presented in the table below. It can be observed that since our proposed CMI constraint effectively provides clearer classification boundaries for the synthetic datasets, thereby offering more valuable guidance information in these real-world applications.



\subsection{Reviewer 2}
We sincerely thank you for the precious time and effort in providing a wealth of suggestions to enhance the quality of our paper. We have carefully read all the comments and provide detailed point-by-point responses as follows. Hopefully, we can adequately address your concerns.

\begin{table}[!ht]
    \centering
    \tabcolsep=10.5pt
    \caption{Performance improvements of CMI constraint on trajectory matching distillation methods.}
    \label{tab:improve_mtt_copy}
    \vspace{-2mm}\resizebox{1\linewidth}{!}{
    \begin{tabular}{l *{6}{c}}
        \toprule
          & \multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{TinyImageNet}  \\
            \midrule
        Method  & 10 & 50 & 10 & 50 & 10 & 50 \\
        \midrule
        MTT   & 65.3$\pm$0.4 & 71.6$\pm$0.2  & 39.7$\pm$0.4 & 47.7$\pm$0.2 & 23.2$\pm$0.2 & 28.0$\pm$0.3  \\
        \textbf{MTT+CMI}  & \textbf{66.7$\pm$0.3} & \textbf{72.4$\pm$0.3}  & \textbf{41.9$\pm$0.4} & \textbf{48.8$\pm$0.2}  & \textbf{24.1$\pm$0.3} & \textbf{28.8$\pm$0.3} \\
        \midrule
        DATM & 66.8$\pm$0.2 & 76.1$\pm$0.3  & 47.2$\pm$0.4 & 54.1$\pm$0.2  & 31.1$\pm$0.3 & 39.7$\pm$0.3 \\
        \textbf{DATM+CMI}  & \textbf{67.4$\pm$0.4}  & \textbf{76.6$\pm$0.1}  & \textbf{47.6$\pm$0.3} & \textbf{55.1$\pm$0.3}  & \textbf{31.9$\pm$0.4} & \textbf{40.6$\pm$0.2}   \\
        \bottomrule
    \end{tabular}}
\end{table}
\subsubsection{Question 1}
\textbf{Additional experiment on more powerful distillation method}

Thanks for the valuable suggestions on improving and completing the experimental aspects. We conduct an additional experiment by applying the CMI constraint on [1]. The experimental results show that our proposed method, as a general-purpose plugin, can achieve performance improvements across various distillation methods.

[1] Towards Lossless Dataset Distillation via Difficulty-Aligned Trajectory Matching. In ICLR, 2024.

\subsubsection{Question 2}
\textbf{Emphasis on the key point of the methodology}

Thank you for your suggestions on improving the presentation. Here, we make a briefly summary of our work as follows: 

On the basis of observing excessive inter-class complexity in the synthetic dataset, i.e., more entangled $\hat{Z}$ when $\mathcal{S}$ is used as the input of a pre-trained classifier $f_{\theta^{*}}$. we introduce conditional mutual information (CMI) from information theory as a metric to evaluate the complexity of the synthetic dataset. By reconstructing the original CMI computation formula in the feature space and incorporating it as a plug-and-play regularization term, which is subsequently minimized, we achieve stable performance improvements across various distillation methods and datasets. A detailed notation is provided in Table below, and we will refine our statements in the final version of the manuscript to ensure greater rigor.

\begin{wraptable}{r}{0.8\linewidth}
    \centering
    % \vspace{-1.5em}
    \caption{Notation. }
    \label{tab:mot}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c |{c}}
        \toprule
         Notation  & Description \\
        \midrule
        $\mathcal{T}$ &  the original training dataset\\
        $\mathcal{S}$ &  the synthetic training dataset\\
        $S$   & the random variable as the input to the network \\
        $Y$  & the random variable as the label\\
        $y$   &  some certain label of the random variable $Y$\\
        $\hat{Z}$ &  the random variable as the penultimate features of the network\\
        $C$  & the number of class \\
        $M$  & the number of the dimensionality of $\hat{Z}$\\
        $f_{\theta^{*}}$  & the pre-trained network \\
        $Q_{\text{emp}}^{y}$  & the empirical center of class $y$\\
        $\lambda$ & the hyper-parameter of CMI constraint\\
        \bottomrule
    \end{tabular}}
    \vspace{-1.0em}
\end{wraptable}
\subsubsection{Question 3}
\textbf{Essential difference with other Information theoretic metrics}

Here, we demonstrate the advantages of CMI over mutual information (MI). In theory, the forward propagation of neural networks $f_{\theta^{*}}$ is a deterministic process, causing $I(X; \hat{Z})$ to degrade into $H(\hat{Z})$, thereby losing its theoretical significance. On the other hand, the value spaces of 
$X$ and $\hat{Z}$ are extremely large, making 
$I(X;\hat{Z})$ very difficult to compute and approximate. As a result, variational methods are commonly employed for estimation, but these estimates are often inaccurate in practice. While CMI enables the computation process to follow a deterministic mathematical expansion by incorporating an additional variable $Y$. This results in a more accurate information metric without the need for additional estimation frameworks (e.g., the contrastive learning framework employed in [2]) and provides a universal regularization approach. The quantitative comparisons with [1] are shown in \textbf{Table 1} provided in \textbf{Sec 5.5}.

[2] MIM4DD: Mutual Information Maximization for Dataset Distillation. In NeurIPS, 2023.


\subsection{Reviewer 3}
Thank you for dedicating your time and effort to reviewing our paper. We are deeply encouraged by your positive comments and recognition of our work. Below, we provide detailed responses to address your concerns.

\subsubsection{Question 1}
\textbf{Limitation and future work}

Thank you for your positive comments and valuable suggestions. Here, we outline some limitations of our proposed method, we will add the corresponding issues in the final version of the manuscript and include them in the future work section.

\textbf{Proxy Model. } Computing CMI requires an proxy model to provide $\hat{Z}$ when $\mathcal{S}$ is used as the input, and selecting an architecture often relies on heuristic methods. 

\textbf{IPC=1. } Minimizing CMI is equal to reduce the Kullback-Leibler (KL) divergence \( D(\cdot \| \cdot) \) between \( P_{S} \) and  \( P_{\hat{Z} \mid y} \), hence, when the IPC is 1, the CMI value is 0. 

Here, we suggest a future direction to better utilize the proxy model; mixing the proxy model discussed in [1] could potentially provide a more informative CMI constraint.

[1] Four eyes see more than two: Dataset Distillation with Mixture-of-Experts. OpenReview Submission, 2024.

\subsection{Reviewer 4}
We would like to express our gratitude for your valuable suggestions and insightful feedback of our paper. Our point-by-point responses are provided below.

\subsubsection{Weakness 1}
\textbf{Contribution of our work}

Thank you for acknowledging the previous work [1] that utilizes conditional mutual information (CMI). Here, we present the distinctions between our proposed method and [1] as follows:

\textbf{Different Optimization Objectives. } [1] lies in the field of knowledge distillation, with the goal of enabling the teacher model to be a better estimated Bayesian classifier. While our proposed method is applied to evaluate the non-linear information between $\mathcal{S}$ and $\hat{Z}$ make the synthetic dataset a more learnable dataset.

\textbf{Different Optimization Intentions. } [1] \textbf{maximize} the CMI value to help the teacher model better capture the contextual information during pre-training phase. In contrast, our proposed method seeks to \textbf{minimize} the CMI value of the synthetic dataset to constrain its complexity during distillation process.

\textbf{Different Optimization Methods. } [1] optimizes by calculating CMI in the probability space, whereas our approach reconstructs the Markov chain (i.e., from $Y \rightarrow X \rightarrow \hat{Y}$ to $Y \rightarrow S \rightarrow \hat{Z}$) in feature space to compute CMI value and validate the theoretical correctness. A stronger constraint effect is achieved as shown in \textbf{Table 7} provided in \textbf{Sec 5.5}.

Beyond that, we emphasize that the derivation process of CMI stems from a \textbf{deterministic} calculation in information theory, that is to say specific calculation is deterministic since the variable is determined. This is why our formulation is similar to [1] (Despite significant differences discussed above). Thus, the focus when applying CMI as a regularization should be why and how to determine the three corresponding random variables.

On the other hand, similar to the way of our work does, a series of studies employing methodologies utilizing information theory to enhance performance across various tasks have been widely applied, including in dataset distillation [2] [3] [4]. In contrast to the various estimation framework necessitated by the \textbf{nondeterministic} calculation of other information metric (e.g., mutual information), we reclaim that the major advantage of CMI is its certainty, i.e., the only estimation derived from the distribution sampling. 

In summary, \textbf{our study is the first to identify the intrinsic class-aware complexity challenge in dataset distillation and to introduce the CMI as a solution}, elucidating its theoretical and practical significance. Furthermore, We offer a novel perspective on how information theory can be effectively applied to this field, thereby highlighting the originality and advancement of our research.

[1] Bayes conditional distribution estimation for knowledge distillation based on conditional mutual information. In ICLR, 2024.

[2] MIM4DD: Mutual Information Maximization for Dataset Distillation. In NeurIPS, 2023.

[3] One Training Fits All: Generalized Data Condensation via Mixture-of-Information Bottleneck Guidance. OpenReview Submission, 2024.

[4] GIFT: Unlocking Full Potential of Labels in Distilled Dataset at Near-zero Cost. Openreview Submission, 2024.

\begin{table}[!ht]
    \centering
    \tabcolsep=12pt
    \caption{Implicit Evaluation of $\hat{Z}$ by Model Accuracy (\%) on CIFAR-10. }
    \label{tab:evaluate_z}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l *{9}{c}}
        \toprule
          & \multicolumn{2}{c}{ConvNet} & \multicolumn{2}{c}{AlexNet} & \multicolumn{2}{c}{ResNet18} & \multicolumn{2}{c}{VGG11}\\
        \midrule
        Method & 10 & 50 & 10 & 50 & 10 & 50 & 10 & 50 \\
        \midrule
         MTT & 98.0 & 100.0 & 97.0 & 99.0 & 98.0 & 100.0 & 100.0 & 100.0\\
         MTT + CMI & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0\\
         \midrule
         DSA & 72.0 & 82.6 & 79.0 & 83.8 & 71.0 & 72.2 & 75.0 & 78.4\\
         DSA + CMI & 100.0 & 100.0 & 99.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0\\
         \midrule
         DM & 47.0 & 87.6 & 59.0 & 85.8 & 56.0 & 79.6 & 60.0 & 78.8\\
         DM + CMI & 99.0 & 100.0 & 98.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0\\
        \bottomrule
    \end{tabular}}
    \vspace{-1.0em}
\end{table}
\subsubsection{Weakness 2}
\textbf{Confusion about the computation of conditional entropy $H(S|\hat{Z}, Y)$}

We truly appreciate your detailed concerns about CMI for enhancing the rigor of the paper. The objective of minimizing the CMI is to mainly reduce the difference between conditional entropy $H(S \mid Y)$ and $H(S \mid \hat{Z}, Y)$,  rather than simply minimizing $H(S \mid \hat{Z}, Y)$. Moreover, introducing additional conditions (i.e., the random variable $\hat{Z}$) will either keep the entropy constant or decrease it, and it cannot lead to an increase as stated. This is a fundamental fact of information theory. 

In fact, $\hat{Z}$ is a function of the random variable $S$, where $S$ serves as the input and $\hat{Z}$ is the output. The function $f_{\theta^{*}}(\cdot)$ is a deterministic function. If the goal is to minimize $H(S \mid \hat{Z}, Y)$, $f_{\theta^{*}}$ should not change any input, leading to $H(S \mid \hat{Z}, Y) = H(S \mid S, Y) = 0$. 

% At this point, when using CMI as a constraint, we acknowledge the existence of the following two conditions. To be clear, we assume $S$ and $Y$ are constants:

% \textbf{Negative. } When $\hat{Z}$ contains completely confused information, such as Gaussian noise. This would \textbf{decrease} the difference between $H(S \mid Y)$ and $H(S \mid \hat{Z}, Y)$ (i.e., CMI).

% \textbf{Positive. } When $\hat{Z}$ contains sufficient class-relevant information. This would also significantly decrease the difference between $H(S \mid Y)$ and $H(S \mid \hat{Z}, Y)$ (i.e., CMI).

At this point, our research lies in the field of dataset distillation, where the optimization objective does not lead to the synthetic dataset becoming entirely noise, which has also been discussed in recent work [5]. To certify this assumption, we used different pre-trained classifier to evaluate the synthetic datasets distilled by different distillation methods as shown in Table below. For a more comprehensive understanding, we also present the performance of CMI constraint using different proxy models in Table.

[5] What is Dataset Distillation Learning? In ICLR, 2024.


\subsubsection{Weakness 3}
\textbf{Ambiguous Expression}

Thank you for pointing out the issue of unclear expression in this section. Here, the point we aim to convey is ``Minimizing the class-aware CMI value constraints the uncertainty brought to $\hat{Z}$ with $\mathcal{S}$ as the input of $f_{\theta^{*}}(\cdot)$'', instead of $H(\hat{Z} \mid \mathcal{S})$. The statement will be revised in the final version of the manuscript to ensure greater precision, and we sincerely appreciate your feedback in pointing this out.

\subsubsection{Weakness 4}
\textbf{Lack of explicit explanation of CMI computation}

Thanks for your suggestion, here, we provide a more detailed mathematical derivation. We first define the input synthetic data $\mathcal{S}$ is conditionally distributed according to $P_{S \mid Y}(\cdot \mid y)$ and mapped into $P_{S} \in \mathcal{P}([M])$. Then we can formulate $P_{\hat{Z} \mid Y}$ as the average of $P_{S}$ with respect to $P_{S \mid Y}(\cdot \mid y)$, which is shown in \textbf{Eq. 5}:
\begin{align} 
    P_{\hat{Z} \mid y } = \mathbb{E}[ P_S \mid Y =y ].
\end{align}
We get the conditional mutual information $I(S ; \hat{Z} \mid Y=y)$ between $S$ and $\hat{Z}$ given $Y$:
\begin{eqnarray}
I(S ; \hat{Z} \mid Y) &=&\sum_{y \in[C]} P_{Y}(y) I(S ; \hat{Z} \mid y)\\
& =&\mathbb{E}\left[D\left(P_S \| P_{\hat{Z} \mid Y}\right) \right].
\end{eqnarray}
Given $Y = y$, the Kullback-Leibler (KL) divergence \( D(\cdot \| \cdot) \) between \( P_{S} \) and  \( P_{\hat{Z} \mid y} \) is equal to \textbf{Eq. 6}:
\begin{eqnarray}
\mathbb{E}\left[D\left(P_{S} \| P_{\hat{Z} \mid y}\right) \mid Y=y\right]
&=&\mathbb{E}\left[\left(\sum_{i=1}^{M} P_{S}(i) \ln \frac{P_{S}(i)}{P_{\hat{Z} \mid y}(\hat{Z}=i \mid Y=y)}\right)\mid Y=y\right]\\
&=&\sum_{S} P_{S \mid Y}(\mathbf{s} \mid y)\left[\sum_{i=1}^{M} P(\hat{Z}=i \mid \mathbf{s})
\ln \frac{P(\hat{Z}=i \mid \mathbf{s})}{P_{\hat{Z} \mid y}(\hat{Z}=i \mid Y=y)}\right],
\end{eqnarray}

These details will be incorporated into the final version of the manuscript to enhance its rigor, and we sincerely appreciate your constructive feedback.

\begin{table}[!ht]
    \centering
    \tabcolsep=10.5pt
    \caption{Performance improvements of CMI constraint on trajectory matching distillation methods.}
    \label{tab:improve_mtt}
    \vspace{-2mm}\resizebox{1\linewidth}{!}{
    \begin{tabular}{l *{6}{c}}
        \toprule
          & \multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{CIFAR100} & \multicolumn{2}{c}{TinyImageNet}  \\
            \midrule
        Method  & 10 & 50 & 10 & 50 & 10 & 50 \\
        \midrule
        MTT   & 65.3$\pm$0.4 & 71.6$\pm$0.2  & 39.7$\pm$0.4 & 47.7$\pm$0.2 & 23.2$\pm$0.2 & 28.0$\pm$0.3  \\
        \textbf{MTT+CMI}  & \textbf{66.7$\pm$0.3} & \textbf{72.4$\pm$0.3}  & \textbf{41.9$\pm$0.4} & \textbf{48.8$\pm$0.2}  & \textbf{24.1$\pm$0.3} & \textbf{28.8$\pm$0.3} \\
        \midrule
        DATM   & 66.8$\pm$0.2 & 76.1$\pm$0.3  & 47.2$\pm$0.4 & 54.1$\pm$0.2  & 31.1$\pm$0.3 & 39.7$\pm$0.3 \\
        \textbf{DATM+CMI}  & \textbf{67.4$\pm$0.4}  & \textbf{76.6$\pm$0.1}  & \textbf{47.6$\pm$0.3} & \textbf{55.1$\pm$0.3}  & \textbf{32.1$\pm$0.4} & \textbf{40.6$\pm$0.2}   \\
        \bottomrule
    \end{tabular}}
\end{table}

\subsubsection{Weakness 5}
\textbf{Comparison with recent SOTA}

Thanks for your suggestion. In contrast to [6] and [7], which are exclusively designed for trajectory matching, (i.e., selecting specific range of trajectories), both our proposed method and the majority baseline methods function as a versatile plugin (e.g., DREAM [8] serves as a universal solution applicable to various distillation methods). Thus, we consider applying the CMI constraint to [6] as suggested by reviewer kma8. As demonstrated in Table below, our proposed approach consistently delivers substantial performance enhancements.

[6] Towards Lossless Dataset Distillation via Difficulty-Aligned Trajectory Matching. In ICLR, 2024.

[7] Prioritize Alignment in Dataset Distillation. In arXiv, 2024.

[8] Dream: Efficient Dataset Distillation by Representative Matching. In ICCV, 2023.

\begin{wraptable}{r}{0.5\linewidth}
    \centering
    % \vspace{-1.5em}
    \caption{Performance improvement with SRe$^2$L on ImageNet-1K. }
    \label{tab:image1k_rebuttal}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l *{3}{c}}
        \toprule
           & \multicolumn{3}{c}{ImageNet-1K} \\
            \midrule
        Method & 10 & 50 & 100\\
        \midrule
        $\text{SRe}^{2}\text{L}$  & 21.3$\pm$0.6 & 46.8$\pm$0.2 & 52.8$\pm$0.3\\
        $\text{SRe}^{2}\text{L}^\dagger$ & 21.5$\pm$0.3 & 46.3$\pm$0.4 & 53.4$\pm$0.1\\
        \textbf{$\text{SRe}^{2}\text{L}$+CMI} & \textbf{24.2$\pm$0.3}  & \textbf{49.1$\pm$0.1} & \textbf{54.6$\pm$0.2}  \\
        \bottomrule
    \end{tabular}}
    \vspace{-1.0em}
\end{wraptable}
\subsubsection{Weakness 6}
\textbf{Details about the implementation of SRe$^2$L}

Thank you for pointing out the confused expression. \textbf{Eq. 3} in our paper represents an abstraction of optimization-based dataset distillation methods, wherein current methods indirectly optimize \textbf{Eq. 2} by aligning specific information (e.g., feature distribution). As discussed in [9] and [10]. instance-based methods (i.e., SRe$^2$L) still falls under this category.

SRe$^2$L optimizes the synthetic dataset by minimizing the loss function $L = l(\phi_{\theta_{\mathcal{T}}}(\mathbf{s}), y)$, where $y \in [C]$ and $l$ represents the cross entropy loss. Due to the instance-independent characteristic of its optimization process, we transit the optimization from the inner loop to the outer loop, enabling simultaneous optimization of the entire synthetic dataset. During the optimization process, synthetic dataset is classified based on predefined labels which are used to compute the loss function, enabling the deployment of CMI constraint. For a fair comparison, we present the impact of altering the loop order in Table below. We attribute the performance improvement to the more precise class boundaries achieved by applying CMI constraint for datasets generated by SRe$^2$L, a critical aspect that has also been emphasized in recent studies [10] [11] [12] [13], and our method can be more easily applied on recent SOTA [12] and [13] with their class-wise supervision.

[9] Generalized Large-Scale Data Condensation via Various Backbone and Statistical Matching. In CVPR, 2024.

[10] Elucidating the Design Space of Dataset Condensation. In NeurIPS, 2024.

[11] Breaking Class Barriers: Efficient Dataset Distillation via Inter-Class Feature Compensator. Openreview Submission, 2024.

[12] Dataset Distillation via the Wasserstein Metric. In arXiv, 2023.

[13] Are Large-scale Soft Labels Necessary for Large-scale Dataset Distillation? In NeurIPS, 2024.

% ### Original Pseudocode

% ```markdown
% for i from 1 to IPC:  # Outer loop optimizes synthetic dataset from 1 to IPC
%     targets = np.arange(1000) # initial hard label
%     for j from 1 to T:  # Inner loop optimizes images from 1 to epoch T
%             Optimize S[i:, ] with L
% ```
% ### Modified Pseudocode
% ```markdown
% targets = np.tile(np.arange(1000), (ipc, 1) )# initial hard label
% for i from 1 to T:  # Outer loop optimizes synthetic dataset from 1 to epoch T
%     for j from 1 to IPC:  # Inner loop optimizes images from 1 to IPC
%         Optimize S[j, :] with L
%     for k from 1 to C:  # apply CMI constraint for each class
%         Optimize S[:, k] with CMI constraint
% ```

